Resource-Aware Session Types for Digital Contracts

Programming digital contracts comes with unique challenges, which include (i) expressing and enforcing protocols of interaction, (ii) controlling resource usage, and (iii) preventing the duplication or deletion of a contract's assets. This article presents the design and type-theoretic foundation of Nomos, a programming language for digital contracts that addresses these challenges. To express and enforce protocols, Nomos is based on shared binary session types. To control resource usage, Nomos employs automatic amortized resource analysis. To prevent the duplication or deletion of assets, Nomos uses a linear type system. A monad integrates the effectful session-typed language with a general-purpose functional language. Nomos' prototype implementation features linear-time type checking and efficient type reconstruction that includes automatic inference of resource bounds via off-the-shelf linear optimization. The effectiveness of the language is evaluated with case studies about implementing common smart contracts such as auctions, elections, and currencies. Nomos is completely formalized, including the type system, a cost semantics, and a transactional semantics to instantiate Nomos contracts on a blockchain. The type soundness proof ensures that protocols are followed at run-time and that types establish sound upper bounds on the resource consumption, ruling out re-entrancy and out-of-gas vulnerabilities.

==> study.tex <==
% \section{Blockchain Applications: A Case Study}
\section{Case Study: Smart Contract Applications}
\label{sec:study}

This section evaluates the design of
Nomos by discussing the implementation of several smart contract
applications and the typical issues that arise.  In particular, we show
\emph{(i)} that session types can enforce the protocol underlying the
ERC-20 token standard, \emph{(ii)} that resource-aware types prevent
out-of-gas exceptions, and \emph{(iii)} that controlled sharing can
prevent common vulnerabilities that are based on
transaction-ordering.

% In particular, we establish that i) session types enforce that the
% tokens on the blockchain meet the ERC-20 token standard,
% ii) resource-aware types detects and prevents out-of-gas exceptions,
% and iii) the acquire-release discipline prevents exploiting
% transaction-order dependent vulnerabilities

\vspace{-0.5em}
\subsection{ERC-20 Token Standard}
Tokens are a representation of a particular asset or utility, that
resides on top of an existing blockchain. ERC-20~\cite{ERC-20}
is a technical standard for smart contracts on the Ethereum blockchain
that defines a common list of standard functions that a token contract
has to implement. The majority of tokens on the Ethereum
blockchain are ERC-20 compliant. The standard requires the following
functions to be implemented:
\begin{itemize}
\item $\m{totalSupply()}$ : returns the total number of tokens in
supply as an integer.

\item $\m{balanceOf(id \; \mi{owner})}$ : returns the account balance of
$\mi{owner}$.

\item $\m{transfer(id \; \mi{to}, int \; \mi{value})}$ : transfers $\mi{value}$
tokens from sender's account to identifier $\mi{to}$.

\item $\m{transferFrom(id \; \mi{from}, id \; \mi{to}, int \; \mi{value})}$ :
transfers $\mi{value}$ number of tokens from identifier $\mi{from}$
to identifier $\mi{to}$.

\item $\m{approve(id \; \mi{spender}, int \; \mi{value})}$ : allows $\mi{spender}$
to withdraw from sender's account up to $\mi{value}$ number of tokens.

\item $\m{allowance(id \; \mi{owner}, id \; \mi{spender})}$ : returns the
number of tokens $\mi{spender}$ is allowed to withdraw from $\mi{owner}$.

\end{itemize}

An ERC-20 token can be declared with the following session type in Nomos:
\begin{tabbing}
$\m{erc20token} = \up \echoice{$\=
$\mb{totalSupply} : \tint \product \down
\m{erc20token},$\\
\>$\mb{balanceOf} : \m{id} \arrow \tint \product \down
\m{erc20token},$\\
\>$\mb{transfer} : \m{id} \arrow \m{id} \arrow \tint \arrow \down
\m{erc20token},$\\
\>$\mb{transferFrom} : \m{id} \arrow \m{id} \arrow \tint \arrow \down
\m{erc20token},$\\
\>$\mb{approve} : \m{id} \arrow \m{id} \arrow \tint \arrow \down
\m{erc20token},$\\
\>$\mb{allowance} : \m{id} \arrow \m{id} \arrow \tint \product \down
\m{erc20token}}$
\end{tabbing}
The type ensures that the token implements the protocol underlying
the ERC-20 standard. To query the total number of
tokens in supply, a client sends the $\m{totalSupply}$ label, and
the contract sends back an integer. If the contract
receives the $\m{balanceOf}$ label followed by the owner's identifier,
it sends back an integer corresponding to the owner's balance. A
balance transfer can be initiated by sending the $\m{transfer}$ label to
the contract followed by sender's and receiver's identifier, and the
amount to be transferred. The $\m{transferFrom}$ label has the same
functionality. If the contract receives $\m{approve}$, it receives the
two identifiers and the value, and updates the allowance internally. Finally, this
allowance can be checked by issuing the $\m{allowance}$ label,
and sending the owner's and spender's identifier.

A programmer can design their own implementation (contract) of the
$\m{erc20token}$ session type. Internally, the contract relies on
custom coins created and named by its owner and used exclusively
for exchanges among private accounts. These coins can be minted
by a special transaction that can only be issued by the owner and that
creates coins out of thin air (consuming gas to create coins).
%
Depending on the functionality intended by the owner, they can employ
different types to represent their coins. For instance, choosing type $\one$, the 
multiplicative unit from linear logic, will allow both creation and destruction
of coins ``for free". A $\mi{mint-one}$ process, typed as $\cdot \vdash
\mi{mint-one} :: (c : \one)$, can create coin $c$ out of thin air (by
closing channel $c$) and a
$\mi{burn-one}$ process, typed as $(c : \one) \vdash \mi{burn-one} ::
(d : \one)$, will destroy the coin $c$ (by waiting on channel $c$).
Nomos' linear type system enforces that the coins are
treated linearly modulo minting and burning. Any transaction that does
not involve minting or burning ensures linearity of these coins.

One specific implementation of the $\m{erc20token}$ session type can be
achieved by storing two lists, one for the balance of each account, and
one for the allowance between each pair of accounts. The account
balance needs to be treated linearly, hence we place this balance list
in the linear context, while we store the allowance list in the functional
context. In this contract, we call the custom coin $\plcoin$, and use
$\plcoins$ to mean $\tlist{\plcoin}$.
The account balance is abstracted using the $\m{account}$
type:
\begin{tabbing}
$\m{account} = \echoice{$\=$\mb{addr} : \m{id} \product \m{account},$
\hspace{8em}\= \% \quad send identifier\\
\>$\mb{add} : \plcoins \lolli \m{account},$
\>\% \quad receive \plcoinsn{} and add internally\\
\>$\mb{subtract} : \tint \arrow \plcoins \tensor \m{account}}$
\>\% \quad receive integer, send \plcoinsn{}
\end{tabbing}
This allows a client to query for the identifier stored in the account,
as well as add and subtract from the account balance. We ignore
the resource consumption as it is not relevant to the example.
The $\mi{balance}$ process provides the $\m{account}$ abstraction.
It internally
stores the identifier in its functional context and \plcoinsn{} in its linear
context, and offers along the linear $\m{account}$ type.
\begin{tabbing}
$(r : \m{id}) \semi (M : \plcoins) \vdash \mi{balance} ::
(acc : \m{account})$
\end{tabbing}
Finally, the contract process stores the allowances as a list of triples
storing the owner's and sender's address and allowance value,
typed as $\m{id} \product \m{id} \product \tint$. Thus, the
$\mi{plcontract}$ process stores the allowance in the functional
context, and the list of accounts in its linear context and offers along
the $\m{erc20token}$ type introduced earlier.
\begin{tabbing}
$(allow : \tlist{\m{id} \product \m{id} \product \tint}) \semi
(accs : \tlist{\m{account}}) \vdash \mi{plcontract} ::
(st : \m{erc20token})$
\end{tabbing}
As an illustration, we show the part of the implementation for initiating a
transfer.
\begin{ntabbing}
\reset
$\procdef{\mi{plcontract} \; allow}{accs}{st} =$ \label{erc-def}\\
\quad \= $\eaccept{lt}{st} \semi$ \label{erc-accept}
\hspace{10em}\=\=\=\% \quad accept a client acquire request\\
\> $\casedef{lt} \ldots$ \label{erc-case}
\>\% \quad switch on label on $lt$\\
\> \quad \= $\mid \labdef{\mb{transfer}}$
\= $\erecvch{lt}{s} \semi$ \label{erc-recv-s}
\>\% \quad receive sender's identifier $s : \m{id}$\\
\>\>\> $\erecvch{lt}{r} \semi$ \label{erc-recv-r}
\>\% \quad receive receiver's identifier $r : \m{id}$\\
\>\>\> $\erecvch{lt}{v} \semi$ \label{erc-recv-v}
\>\% \quad receive transfer value $v : \tint$\\
\>\>\> $\edetach{st}{lt} \semi$ \label{erc-detach}
\>\% \quad detach from client\\
\>\>\> $\ldots$ \label{ecr-code1}
\>\% \quad extract sender and receiver's account \ldots\\
\>\>\> $\ldots$ \label{ecr-code1}
\>\% \quad and store in $sa$ and $ra$ resp.\\
\>\>\> $\esendl{sa}{\mb{subtract}} \semi$ \label{erc-sub}
\>\% \quad subtract \plcoinsn{} corresponding to \ldots\\
\>\>\> $\esendl{sa}{v} \semi$ \label{erc-send-v}
\>\% \quad $v$ from account channel $sa$\\
\>\>\> $\erecvch{sa}{m}$ \label{erc-recv-m}
\>\% \quad receive transfer amount $m$\\
\>\>\> $\esendl{ra}{\mb{add}} \semi$ \label{erc-add}
\>\% \quad add $m : \plcoins$ to \ldots\\
\>\>\> $\esendch{ra}{m} \semi$ \label{erc-send-m}
\>\% \quad account channel $ra$\\
\>\>\> $\procdef{\mi{plcontract} \; allow}{accs}{st}$
\label{erc-recurse}
\end{ntabbing}
The contract first receives the sender and receiver's identifiers
(lines~\ref{erc-recv-s} and \ref{erc-recv-r}) and the transfer
value $v$. The contract then detaches from the client (line
\ref{erc-detach}). We skip the code of extracting the sender's
and receiver's account from the list $accs$ and store them
in $sa$ and $ra$ of type $\m{account}$, respectively. The
contract then subtracts the \plcoinsn{} from account $sa$
(lines~\ref{erc-sub} and \ref{erc-send-v}) and receives and
stores them in $m$ (line~\ref{erc-recv-m}). This balance is then
added to $ra$'s account (lines~\ref{erc-add} and \ref{erc-send-m}).
An important point here is that Nomos enforces linearity
of the transfer transaction. Since $m : \plcoins$ is typed
as a linear asset, it cannot be discarded or modified. The
amount deducted from sender must be transferred to the receiver
(since no minting is involved here).

\paragraph{\textbf{\textit{Hacker Gold (HKG) Token}}}
The HKG token is one particular implementation of the ERC-20
token specification. Recently, a vulnerability was discovered
in the HKG token smart contract based on a typographical
error leading to a re-issuance of the entire token~\cite{HKG-News}.

The typographical error in the contract came about when updating the
receiver's balance during a transfer. Instead of
writing $\lstinline{balance += value}$, the programmer mistakenly
wrote $\lstinline{balance =+ value}$ (semantically meaning
$\lstinline{balance = value}$). Moreover, while testing
this error was missed, because the first transfer always succeeds
(since the two statements are semantically equivalent when
$\lstinline{balance = 0}$). Nomos' type system would have
caught the linearity violation in the latter statement that
drops the existing balance in the recipient's account.

\vspace{-0.5em}
\subsection{Out-of-Gas Vulnerabilities}
A broad family of contract vulnerabilities concerns \emph{out-of-gas}
behavior. This section describes some common
patterns causing such vulnerabilities with examples and evaluates
Nomos' ability to detect them. 
%
As mentioned before, gas is the fuel of computation in several
blockchains such as Ethereum that users provide together with a
transaction.  If the computation exceed its allotted amount of gas, an
out-of-gas exception is raised and the transaction is aborted. A
contract that does not correctly handle the possible abortion of a
transaction is at risk of a gas-focused vulnerability. The examples
presented have been inspired from prior work~\cite{MadMax-OOPSLA18}.

\paragraph{\textbf{\textit{Unbounded Mass Operations}}}
This can be caused by a loop
whose iterations cannot be bounded at design time because they
depend on the user input or the state of the contract.
%
Such a loop can become economically too expensive to perform or even
exceed the \emph{block gas limit}, which would make the contract
unusable in Ethereum. 
%
Consider the contract snippet below in Solidity.
%\jan{can we remove the syntax
%  highlighting? There is a nice auction example here
%  https://github.com/ethereum/wiki/wiki/Safety}
\begin{lstlisting}[basicstyle=\small\ttfamily, language=Solidity,
columns=fullflexible]
function applyInterest() returns (uint) {
  for (uint i = 0; i < accounts.length; i++)
    // apply 5 percent interest
    accounts[i].balance = accounts[i].balance * 105 / 100;
  return accounts.length; }
\end{lstlisting}
As the number of accounts increases, the gas requirement for
$\m{applyInterest}$ rises. If an attacker can control the number of
accounts then this loop can be used for a \emph{denial-of-service} attack.

Nomos can infer the linear gas cost for $\m{applyInterest}$.
Suppose the gas cost for executing one loop iteration is $c$
(ignoring other constant costs). Nomos will assign the resource-aware
type $\plist{\tint}{c}$ to the variable $\m{accounts}$, assigning a potential of $c$
to each element in the list, which is consumed to perform each
loop iteration. Such \emph{gas sharing schemes} would be sufficient to reimburse all
unsuccessful participants in an auction and proved sound by a
resource-aware type derivation. The onus of supplying the gas cost for executing
the loop does not fall on one user, and is amortized over all users
of the contract. This avoid the denial-of-service vulnerability of
this contract.

Nomos also supports more complex gas sharing schemes that would allow
a function like $\m{applyInterest}$ to be executed an unlimited number
of times. One possibility would be to internally store the accounts in
two lists.  The list of \emph{active accounts} would have type
$\plist{\tint}{c}$ and carry potential $c$ per element to cover the
cost of adding interest.  The list of \emph{inactive accounts} would
have type $\plist{\tint}{0}$ and not carry potential.  The function
$\m{applyInterest}$ would operate only on the active accounts and move
all accounts to the inactive list during its iteration.  The contract
would allow users to move their account back to the active list,
charging the additional gas cost $c$ to pay for the potential of the
additional list element.  Again, the type system would prove that the
gas cost of each transaction is indeed constant.

\paragraph{\textbf{\textit{Non-Isolated External Calls}}}
A contract may also have out-of-gas vulnerabilities because it is invoking an
external function that may throw an out-of-gas
exception. This occurs when a programmer has not considered
an external call extensively, as is often the case with implicit
calls. For instance, on the Ethereum blockchain, sending Ether
involves calling a fallback function on the recipient's side. All it
takes for an attacker is to provide a fallback function that runs out
of gas.

All calls in Nomos, whether internal within the same account
or external, are checked for sufficient potential. The type of
a function (on the turnstile, and the potential of the arguments)
indicates precisely the gas cost of the function call. The caller
must have enough potential for both the call and the continuation
that handles the result of the call. This is expressed, for instance,
in the $\{\}E_{PP}$ rule in Figure~\ref{fig:typing-functional}, where
$p$ is the potential for the call, and $q$ is the potential for the
continuation. Type checking guarantees that any function
implementation does not run out of gas during execution, thus
protecting all external calls against this out-of-gas vulnerability.

\vspace{-0.5em}
\subsection{Transaction-Ordering Dependence}
A common source of security bugs in smart contracts is when they
depend on the order in which the transactions are executed in
the contract.
Consider a scenario where a blockchain is in some state
and a new added block contains two transactions
invoking the same contract. In such a scenario,
users have uncertain knowledge of which state the contract is
at when their individual invocation is executed. Only the miner
who mines the new block can decide the order of the transactions.
If the outcome of either of the two transactions depends on the
order in which they are executed, then the contract suffers from a
transaction-order dependent vulnerability.

Consider a puzzle contract~\cite{Oyente-CCS16}
which rewards users who solve
a computational puzzle and submit the solution to the contract.
The contract allows two functions, one that allows the owner
to update the reward, and the other that allows a user to submit
their solution and collect winnings. The following code presents
the relevant aspects of the implementation in Solidity.
\begin{lstlisting}[basicstyle=\small\ttfamily, language=Solidity,
columns=fullflexible]
contract Puzzle {
  ...
  address public owner;					// contract owner
  uint public reward;							// reward value
  ...
  function update() {
    if (msg.sender == owner){
      owner.send(reward);												// owner sends reward to contract
      reward = msg.value; }}
  ...
  function submit(){
    if (verify(msg.data)) {										// verify the solution
      msg.sender.send(reward); }}}			// send reward to user
\end{lstlisting}

A malicious owner of the contract can listen on the network to
check for users submitting solutions to the contract. If they encounter
such a transaction, they can issue their own $\m{update}$ transaction
to update the reward and make it 0 (or a smaller amount). With a
certain chance, the $\m{update}$ transaction can execute before
the $\m{submit}$, and the owner can enjoy a free solution to the
puzzle. Thus, the transaction-order dependency can be exploited.

In Nomos, the contract can be implemented to offer the following type
\begin{tabbing}
$\m{puzzle} = \up \echoice{$
\=$\mb{update} : \m{id} \arrow \m{money} \lolli \down \m{puzzle},$\\
\>$\mb{submit} : \tint \product \echoice{$
\=$\mb{success} : \m{solution} \arrow \m{money} \tensor \down
\m{puzzle},$\\
\>\>$\mb{failure} : \down \m{puzzle}}}$
\end{tabbing}
The contract still supports the two transactions, one to update the
reward, where it receives the identifier, verifies that the sender is
the owner, receives money from the sender, and terminates the
session. The transaction to submit a solution has a \emph{guard}
associated with it. First, the contract sends an integer corresponding
to the reward amount, the user then verifies that the reward matches
the expected reward (the guard condition). If the guard succeeds,
the user sends the $\m{success}$ label, followed by the solution,
receives the winnings, and the session terminates. If the guard
fails, the user issues the $\m{failure}$ label and immediately
terminates the session.

The acquire-release discipline along with the guarded transaction
prevents the exploitation of the ordering dependent vulnerability.
Since the user \emph{acquires} the contract before submitting
the solution, the user holds exclusive access to the contract data.
This data cannot be modified by any other user, even the owner
of the contract during this \emph{critical section}. Thus, if the
guard condition succeeds, the user is guaranteed to receive
their expected winnings.

%%% Local Variables:
%%% mode: latex
%%% mode: flyspell
%%% TeX-master: "icfp19.tex"
%%% End:

